Milky Way Satellite Census. III. Constraints on Dark Matter Properties from Observations of Milky Way Satellite Galaxies

We perform a comprehensive study of Milky Way (MW) satellite galaxies to constrain the fundamental properties of dark matter (DM). This analysis fully incorporates inhomogeneities in the spatial distribution and detectability of MW satellites and marginalizes over uncertainties in the mapping between galaxies and DM halos, the properties of the MW system, and the disruption of subhalos by the MW disk. Our results are consistent with the cold, collisionless DM paradigm and yield the strongest cosmological constraints to date on particle models of warm, interacting, and fuzzy dark matter. At $95\%$ confidence, we report limits on (i) the mass of thermal relic warm DM, $m_{\rm WDM} > 6.5\ \mathrm{keV}$ (free-streaming length, $\lambda_{\rm{fs}} \lesssim 10\,h^{-1}\ \mathrm{kpc}$), (ii) the velocity-independent DM-proton scattering cross section, $\sigma_{0} < 8.8\times 10^{-29}\ \mathrm{cm}^{2}$ for a $100\ \mathrm{MeV}$ DM particle mass (DM-proton coupling, $c_p \lesssim (0.3\ \mathrm{GeV})^{-2}$), and (iii) the mass of fuzzy DM, $m_{\phi}> 2.9 \times 10^{-21}\ \mathrm{eV}$ (de Broglie wavelength, $\lambda_{\rm{dB}} \lesssim 0.5\ \mathrm{kpc}$). These constraints are complementary to other observational and laboratory constraints on DM properties.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar

# Primary file names
main=main
out=y3-mw-sats-dm
reply=reply
outline=outline
filename=${main}

# LATEX environment variables
export TEXINPUTS:=.:./texmf//:./tables/:./tex:./tex/texmf//:./tex/tables/:
export BSTINPUTS:=.:./texmf/bib/:./tex:./tex/texmf/bib/:

# Document class switcher flags
#aastex=\def\flag{aastex}\def\authlist{authors_aastex}
#revtex=\def\flag{revtex}\def\authlist{authors_revtex}
#apjtex=\def\flag{emulateapj}\def\authlist{authors_aastex}
#arxiv=\def\flag{emulateapj}\def\authlist{authors_aastex}

# Submission flags
submit=${apjtex}
#draft=${aastex}\def\linenums{\linenumbers}
draft=${apjtex}\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir=tar
figdir=./figures
figures=$(figdir)/*.pdf $(figdir)/*.png
tabdir=./tables
tables=$(tabdir)/*.tex
#stydir=./texmf
#styles=$(stydir)/styles/*.{sty,cls}
styles=aastex61.cls apj.bst
source=$(main).{bbl,bib} commands.tex authors.tex ack.tex

tarfiles=$(figures) $(tables) $(styles) $(source)

all: export flag = ${draft}
all: main copy

copy: 
	cp $(filename).pdf $(out).pdf

touch:
	touch ${filename}.tex

# http://stackoverflow.com/q/8028314/
TARGETS=aastex apj emulateapj
$(TARGETS): export flag = \def\flag{$(@)}
$(TARGETS): 
	$(MAKE) -e main
	$(MAKE) -e tar

TARGETS=draft submit arxiv
$(TARGETS): export flag = ${$(@)}
$(TARGETS): 
	$(MAKE) -e main
	$(MAKE) -e tar

main :
	latexmk -pdf "${filename}"

pdflatex :
	pdflatex "${flag}\input{${filename}}"
	bibtex ${filename}||true
	pdflatex "${flag}\input{${filename}}"
	pdflatex "${flag}\input{${filename}}"

tar : 
	mkdir -p $(tardir)
	cp $(filename).tex $(tardir)
	echo $(tarfiles)
	cp $(tarfiles) $(tardir)
	cp $(filename).pdf $(tardir)/$(out).pdf
	cd $(tardir) && tar -czf ../$(out).tar.gz . && cd ..
	rm -rf $(tardir)

reply : filename=${reply}
reply : flag=${draft}
reply : main

outline : filename=${outline}
outline : flag=${draft} 
outline : main

clean:
	rm -f *.ps ${filename}.pdf *.log *.aux *.out *.dvi *.bbl *.blg *Notes.bib *.synctex.gz *.fdb_latexmk *.fls


